Retrieval-Enhanced Contrastive Vision-Text Models

Contrastive image-text models such as CLIP form the building blocks of many state-of-the-art systems. While they excel at recognizing common generic concepts, they still struggle on fine-grained entities which are rare, or even absent from the pre-training dataset. Hence, a key ingredient to their success has been the use of large-scale curated pre-training data aiming at expanding the set of concepts that they can memorize during the pre-training stage. In this work, we explore an alternative to encoding fine-grained knowledge directly into the model's parameters: we instead train the model to retrieve this knowledge from an external memory. Specifically, we propose to equip existing vision-text models with the ability to refine their embedding with cross-modal retrieved information from a memory at inference time, which greatly improves their zero-shot predictions. Remarkably, we show that this can be done with a light-weight, single-layer, fusion transformer on top of a frozen CLIP. Our experiments validate that our retrieval-enhanced contrastive (RECO) training improves CLIP performance substantially on several challenging fine-grained tasks: for example +10.9 on Stanford Cars, +10.2 on CUB-2011 and +7.3 on the recent OVEN benchmark, where we even outperform the fine-tuned models on unseen classes.

==> discussion.tex <==
\vspace{-0.2cm}
\section{Limitations}

\vspace{-0.2cm}
\head{Access to a large and rich memory.}
The main limitation of this work is that it supposes that one has access to a large and rich source of knowledge, the memory of image and text pairs.
While we have shown that large public dataset such as LAION can serve this purpose, the best of performance is obtained with a large private memory.
Ideally, one could use search engine APIs as the memory.

\vspace{-0.2cm}
\head{Compute efficiency.}
Our method shows important gains of performance in zero-shot transfer compared to CLIP, \ie our backbone model.
However, this comes at the cost of an increase of inference time.
In practice, we use a highly-optimized approximate $k$-NN algorithm~\cite{guo2020accelerating}, and querying $1$B examples in Webli takes milliseconds.
It is also possible to mitigate this issue by reducing the number of retrieved items, as shown in Figure~\ref{fig:ablation}.
Indeed, retrieving a single element already improves over CLIP with a non-trivial margin (+7.1 absolute points on Cars dataset) while reducing substantially the compute requirements compared to our best performing model.

% While we have shown important gains of performance in zero-shot transfer compared to the original vision-text encoders that our method is build on, this comes at the cost of an increase of inference time.
% A solution to mitigate this effect is to reduce the number of retrieved items, as shown in Figure~\ref{fig:ablation}.
% Indeed, retrieving a single element already improves over CLIP with a non-trivial margin (+7.1 absolute points on Cars dataset) while reducing substantially the compute requirements compared to our best performing model.

